Fermat's Last Theorem for regular primes

We formalise the proof of the first case of Fermat's Last Theorem for regular primes using the \emph{Lean} theorem prover and its mathematical library \emph{mathlib}. This is an important 19th century result that motivated the development of modern algebraic number theory. Besides explaining the mathematics behind this result, we analyze in this paper the difficulties we faced in the formalisation process and how we solved them. For example, we had to deal with a diamond about characteristic zero fields and problems arising from multiple nested coercions related to number fields. We also explain how we integrated our work to \emph{mathlib}.

==> lstlean2.tex <==
% Listing style definition for the Lean Theorem Prover.
% Defined by Jeremy Avigad, 2015, by modifying Assia Mahboubi's SSR style.
% Unicode replacements taken from Olivier Verdier's unixode.sty

\lstdefinelanguage{lean} {
	
	% Anything betweeen $ becomes LaTeX math mode
	%mathescape=true,
	% Comments may or not include Latex commands
	texcl=false,
	
	% keywords, list taken from lean-syntax.el
	morekeywords=[1]{
		import, prelude, protected, private, noncomputable, definition, meta, renaming,
		hiding, exposing, parameter, parameters, begin, conjecture, constant, constants,
		hypothesis, lemma, corollary, variable, variables, premise, premises, theory,
		print, theorem, proposition, example, abstract,
		open, as, export, override, axiom, axioms, inductive, with, without,
		structure, record, universe, universes,
		alias, help, precedence, reserve, declare_trace, add_key_equivalence,
		match, infix, infixl, infixr, notation, postfix, prefix, instance,
		eval, vm_eval, check, coercion, end, this, suppose,
		using, using_well_founded, namespace, section, fields,
		attribute, local, set_option, extends, include, omit, classes, class,
		instances, coercions, attributes, raw, replacing,
		calc, have, show, suffices, by, in, at, let, forall, Pi, fun,
		exists, if, dif, then, else, assume, take, obtain, from, aliases, register_simp_ext,
		mutual, def, run_command
	},
	
	% Sorts
	morekeywords=[2]{Type, Prop, Type*, Type₀, Type₁, Type₂, Type₃},
	
	% tactics, list taken from lean-syntax.el
	% morekeywords=[3]{
		% Cond, or_else, then, try, when, assumption, eassumption, rapply,
		% apply, fapply, eapply, rename, intro, intros, all_goals, fold, focus, focus_at,
		% generalize, generalizes, clear, clears, revert, reverts, back, beta, done, exact, rexact,
		% refine, repeat, whnf, rotate, rotate_left, rotate_right, inversion, cases, rewrite,
		% xrewrite, krewrite, blast, simp, esimp, unfold, change, check_expr, contradiction,
		% exfalso, split, existsi, constructor, fconstructor, left, right, injection, congruence, reflexivity,
		% symmetry, transitivity, state, induction, induction_using, fail, append,
		% substvars, now, with_options, with_attributes, with_attrs, note
		% },
	
	% modifiers, taken from lean-syntax.el
	% note: 'otherkeywords' is needed because these use a different symbol.
	% this command doesn't allow us to specify a number -- they are put with [1]
	% otherkeywords={
		% [persistent], [notation], [visible], [instance], [trans_instance],
		% [class], [parsing-only], [coercion], [unfold_full], [constructor],
		% [reducible], [irreducible], [semireducible], [quasireducible], [wf],
		% [whnf], [multiple_instances], [none], [decl], [declaration],
		% [relation], [symm], [subst], [refl], [trans], [simp], [congr], [unify],
		% [backward], [forward], [no_pattern], [begin_end], [tactic], [abbreviation],
		% [reducible], [unfold], [alias], [eqv], [intro], [intro!], [elim], [grinder],
		% [localrefinfo], [recursor]
		% },
	
	% Various symbols
	literate=
	{α}{{\ensuremath{\mathrm{\alpha}}}}1
	{β}{{\ensuremath{\mathrm{\beta}}}}1
	{γ}{{\ensuremath{\mathrm{\gamma}}}}1
	{δ}{{\ensuremath{\mathrm{\delta}}}}1
	{ε}{{\ensuremath{\mathrm{\varepsilon}}}}1
	{ζ}{{\ensuremath{\mathrm{\zeta}}}}1
	{η}{{\ensuremath{\mathrm{\eta}}}}1
	{θ}{{\ensuremath{\mathrm{\theta}}}}1
	{ι}{{\ensuremath{\mathrm{\iota}}}}1
	{κ}{{\ensuremath{\mathrm{\kappa}}}}1
	{μ}{{\ensuremath{\mathrm{\mu}}}}1
	{ν}{{\ensuremath{\mathrm{\nu}}}}1
	{ξ}{{\ensuremath{\mathrm{\xi}}}}1
	{π}{{\ensuremath{\mathrm{\mathnormal{\pi}}}}}1
	{ρ}{{\ensuremath{\mathrm{\rho}}}}1
	{σ}{{\ensuremath{\mathrm{\sigma}}}}1
	{τ}{{\ensuremath{\mathrm{\tau}}}}1
	{φ}{{\ensuremath{\mathrm{\varphi}}}}1
	{χ}{{\ensuremath{\mathrm{\chi}}}}1
	{ψ}{{\ensuremath{\mathrm{\psi}}}}1
	{ω}{{\ensuremath{\mathrm{\omega}}}}1
	
	{Γ}{{\ensuremath{\mathrm{\Gamma}}}}1
	{Δ}{{\ensuremath{\mathrm{\Delta}}}}1
	{Θ}{{\ensuremath{\mathrm{\Theta}}}}1
	{Λ}{{\ensuremath{\mathrm{\Lambda}}}}1
	{Σ}{{\ensuremath{\mathrm{\Sigma}}}}1
	{Φ}{{\ensuremath{\mathrm{\Phi}}}}1
	{Ξ}{{\ensuremath{\mathrm{\Xi}}}}1
	{Ψ}{{\ensuremath{\mathrm{\Psi}}}}1
	{Ω}{{\ensuremath{\mathrm{\Omega}}}}1
	{$}{{\ensuremath{\$}}}1
	
	{ℵ}{{\ensuremath{\aleph}}}1
	{��}{{\ensuremath{\mathcal{N}}}}1
	
	{≤}{{\ensuremath{\leq}}}1
	{≥}{{\ensuremath{\geq}}}1
	{≠}{{\ensuremath{\neq}}}1
	{≈}{{\ensuremath{\approx}}}1
	{≡}{{\ensuremath{\equiv}}}1
	{≃}{{\ensuremath{\simeq}}}1
	
	{≤}{{\ensuremath{\leq}}}1
	{≥}{{\ensuremath{\geq}}}1
	
	{∂}{{\ensuremath{\partial}}}1
	{∆}{{\ensuremath{\triangle}}}1 % or \laplace?
	
	{∫}{{\ensuremath{\int}}}1
	{∑}{{\ensuremath{\mathrm{\Sigma}}}}1
	{Π}{{\ensuremath{\mathrm{\Pi}}}}1
	
	{⊥}{{\ensuremath{\perp}}}1
	{∞}{{\ensuremath{\infty}}}1
	{∂}{{\ensuremath{\partial}}}1
	
	{∓}{{\ensuremath{\mp}}}1
	{±}{{\ensuremath{\pm}}}1
	{×}{{\ensuremath{\times}}}1
	
	{⊕}{{\ensuremath{\oplus}}}1
	{⊗}{{\ensuremath{\otimes}}}1
	{⊞}{{\ensuremath{\boxplus}}}1
	
	{∇}{{\ensuremath{\nabla}}}1
	{√}{{\ensuremath{\sqrt}}}1

	
	{⬝}{{\ensuremath{\cdot}}}1
	{•}{{\ensuremath{\cdot}}}1
	{∘}{{\ensuremath{\circ}}}1
	
	%{⁻}{{\ensuremath{^{\textup{\kern1pt\rule{2pt}{0.3pt}\kern-1pt}}}}}1
	{⁻}{{\ensuremath{^{-}}}}1
	{▸}{{\ensuremath{\blacktriangleright}}}1
	
	{∧}{{\ensuremath{\wedge}}}1
	{∨}{{\ensuremath{\vee}}}1
	{¬}{{\ensuremath{\neg}}}1
	{⊢}{{\ensuremath{\vdash}}}1
	
	%{⟨}{{\ensuremath{\left\langle}}}1
	%{⟩}{{\ensuremath{\right\rangle}}}1
	{⟨}{{\ensuremath{\langle}}}1
	{⟩}{{\ensuremath{\rangle}}}1
	
	{↦}{{\ensuremath{\mapsto}}}1
	{→}{{\ensuremath{\rightarrow}}}1
	{↔}{{\ensuremath{\leftrightarrow}}}1
	{⇒}{{\ensuremath{\Rightarrow}}}1
	{⟹}{{\ensuremath{\Longrightarrow}}}1
	{⇐}{{\ensuremath{\Leftarrow}}}1
	{⟸}{{\ensuremath{\Longleftarrow}}}1
	
	{∩}{{\ensuremath{\cap}}}1
	{∪}{{\ensuremath{\cup}}}1
	{⊂}{{\ensuremath{\subseteq}}}1
	{⊆}{{\ensuremath{\subseteq}}}1
	{⊄}{{\ensuremath{\nsubseteq}}}1
	{⊈}{{\ensuremath{\nsubseteq}}}1
	{⊃}{{\ensuremath{\supseteq}}}1
	{⊇}{{\ensuremath{\supseteq}}}1
	{⊅}{{\ensuremath{\nsupseteq}}}1
	{⊉}{{\ensuremath{\nsupseteq}}}1
	{∈}{{\ensuremath{\in}}}1
	{∉}{{\ensuremath{\notin}}}1
	{∋}{{\ensuremath{\ni}}}1
	{∮}{{\ensuremath{\oint}}}1
	{∌}{{\ensuremath{\notni}}}1
	{∅}{{\ensuremath{\emptyset}}}1
	{$}{{\ensuremath{\textdollar}}}1
	{∖}{{\ensuremath{\setminus}}}1
	{†}{{\ensuremath{\dag}}}1
	{⁺}{{\ensuremath{^+}}}1
	{|}{{\ensuremath{\mid}}}1
	{∣}{{\ensuremath{\mid}}}1
	{ℕ}{{\ensuremath{\mathbb{N}}}}1
	{ℤ}{{\ensuremath{\mathbb{Z}}}}1
	{ℝ}{{\ensuremath{\mathbb{R}}}}1
	{ℚ}{{\ensuremath{\mathbb{Q}}}}1
	{ℂ}{{\ensuremath{\mathbb{C}}}}1
	{⌞}{{\ensuremath{\llcorner}}}1
	{⌟}{{\ensuremath{\lrcorner}}}1
	{⦃}{{\ensuremath{\{\!|}}}1
	{⦄}{{\ensuremath{|\!\}}}}1
	{ℍ}{{\ensuremath{\mathbb{H}}}}1
	{��}{{\ensuremath{\mathcal{J}}}}1
	{₁}{{\ensuremath{_1}}}1
	{₂}{{\ensuremath{_2}}}1
	{₃}{{\ensuremath{_3}}}1
	{₄}{{\ensuremath{_4}}}1
	{₅}{{\ensuremath{_5}}}1
	{₆}{{\ensuremath{_6}}}1
	{₇}{{\ensuremath{_7}}}1
	{₈}{{\ensuremath{_8}}}1
	{₉}{{\ensuremath{_9}}}1
	{₀}{{\ensuremath{_0}}}1
	{ᵢ}{{\ensuremath{_i}}}1
	
	{¹}{{\ensuremath{^1}}}1
	{ˣ}{{\ensuremath{^{\times}}}}1
	{ₙ}{{\ensuremath{_n}}}1
	{ₘ}{{\ensuremath{_m}}}1
	{↑}{{\ensuremath{\uparrow}}}1
	{↓}{{\ensuremath{\downarrow}}}1
	
	{▸}{{\ensuremath{\triangleright}}}1
	
	{Σ}{{\color{symbolcolor}\ensuremath{\Sigma}}}1
	{Π}{{\color{symbolcolor}\ensuremath{\Pi}}}1
	{∀}{{\color{symbolcolor}\ensuremath{\forall}}}1
	{∃}{{\color{symbolcolor}\ensuremath{\exists}}}1
	{λ}{{\color{symbolcolor}\ensuremath{\mathrm{\lambda}}}}1
	
	{:=}{{\color{symbolcolor}:=}}1
	{=}{{\color{symbolcolor}=}}1
	{<}{{\color{symbolcolor}<}}1
	{+}{{\color{symbolcolor}+}}1
	{*}{{\color{symbolcolor}*}}1,
	
	% Comments
	%comment=[s][\itshape \color{commentcolor}]{/-}{-/},
	morecomment=[s][\color{commentcolor}]{/-}{-/},
	morecomment=[l][\itshape \color{commentcolor}]{--},
	
	% Spaces are not displayed as a special character
	showstringspaces=false,
	
	% keep spaces
	keepspaces=true,
	
	% String delimiters
	morestring=[b]",
	morestring=[d],
	
	% Size of tabulations
	tabsize=3,
	
	% Enables ASCII chars 128 to 255
	extendedchars=true,
	
	% Case sensitivity
	sensitive=true,
	
	% Automatic breaking of long lines
	breaklines=true,
	
	% Default style fors listingsred
	basicstyle=\ttfamily,
	
	% Position of captions is bottom
	captionpos=b,
	
	% Full flexible columns
	columns=[l]fullflexible,
	
	
	% Style for (listings') identifiers
	identifierstyle={\ttfamily\color{black}},
	% Note : highlighting of Coq identifiers is done through a new
	% delimiter definition through an lstset at the begining of the
	% document. Don't know how to do better.
	
	% Style for declaration keywords
	keywordstyle=[1]{\ttfamily\color{keywordcolor}},
	
	% Style for sorts
	keywordstyle=[2]{\ttfamily\color{sortcolor}},
	
	% Style for tactics keywords
	% keywordstyle=[3]{\ttfamily\color{tacticcolor}},
	
	% Style for attributes
	% keywordstyle=[4]{\ttfamily\color{attributecolor}},
	
	% Style for strings
	stringstyle=\ttfamily,
	
	% Style for comments
	% commentstyle={\ttfamily\footnotesize },
	
}
